Securely Trading Unverifiable Information without Trust

In future, information may become one of the most important assets in economy. However, unlike common goods (e.g. clothing), information is troublesome in trading since the information commodities are \emph{vulnerable}, as they lose their values immediately after revelation, and possibly unverifiable, as they can be subjective. By authorizing a trusted center (e.g. Amazon) to help manage the information trade, traders are ``forced'' to give the trusted center the ability to become an information monopolist. To this end, we need a trust-free (i.e. without a trusted center and with only strategic traders) unverifiable information trade protocol such that it 1) motivates the sellers to provide high quality information, and the buyer to pay for the information with a fair price (truthful); 2) except the owner, the information is known only to its buyer if the trade is executed (secure). In an unverifiable information trade scenario (e.g. a medical company wants to buy experts' opinions on multiple difficult medical images with unknown pathological truth from several hospitals), we design a trust-free, truthful, and secure protocol, Smart Info-Dealer (SMind), for information trading, by borrowing three cutting-edge tools that include peer prediction, secure multi-party computation, and smart contract. With SMind, without a trusted center, a seller with high-quality information is able to sell her information securely at a fair price and those with low-quality information cannot earn extra money with poor information or steal information from other sellers. We believe SMind will help describe a free and secure information trade scenario in the future.

==> former-proof.tex <==
\section{Formal security proof: Preliminaries}\label{Appendix:securityproof}
%roadmap


\subsection{Cryptographic definitions and building blocks}

\ym{GUC secure enc + commitment, UC secure MPC/GUC secure 2PC}


\begin{definition}(negligible function)\par
A function $\mu: \mathbbm{N} \rightarrow \mathbbm{R}$ is \textit{negligible} iff $ \forall c\in \mathbbm{N}, \exists n_0 \in \mathbbm{N} $ such that $\forall n\ge n_0, \mu(n)\le n^{-c}$.
\end{definition}


\paragraph{Commitment scheme }

For provable security reasons, we use hash function modeled as random oracle to substitute commitment scheme. It is described as follows:\par
$Commit(m,r) = H(r\|m)$\par
$Verify(c,m,r) = \mathbbm{I}_{\{H(r\| m ) = c\}}$


\subsection{Simulation Proof Techniques}
We first introduce the standard cryptographic notion - basic UC framework and generalized UC framework in a high-level way, then we present some details to provide a basis of the proof in next section.\par

\ym{Notation}

\subsubsection{Basic UC framework}
We denote $\pi$ as an \textit{implementation} (such as actual real-world protocol) and $\phi$ is a \textit{specification} (such as the functionality that we wish to implement is securely computed directly by a trusted agent). We denote them ($\pi$ and $\phi$) as \textit{challenge protocols}.\par
The intuition behind the basic UC framework is that any adversary $\mathcal{A}$ attacking the protocol $\pi$ should learn no more information that could have been obtained via the use of a simulator $\mathcal{S}$ attacking a protocol $\phi$.
Furthermore, we would like this property to be maintained even if $\phi$ is used as a subroutine of arbitrary other protocols.\par
Therefore, \cite{canetti2001universally} induced a distinguisher environment $\mathcal{Z}$ that is tasked to distinguish between actual attacks on protocol $\pi$, and and simulated attacks on protocol. $\mathcal{Z}$ is empowered to control the inputs supplied to the parties running the protocol, and observe the parties' outputs at all stages during the protocol execution. Adversarial attacks is orchestrated and monitored by a $\mathcal{Z}$.\par
Using environment $\mathcal{Z}$, we restate the distinguishing notion as follows. The environment $\mathcal{Z}$ intends to distinguish between adversarial attacks prepetrated by $\mathcal{A}$ on protocol $\pi$, and attack simulations conducted by $\mathcal{S}$ with protocol $\phi$. If no environment can successfully distinguish these two possible scenarios, then
protocol $\pi$ is said to \textit{UC emulate} the protocol $\phi$.\par
The \textit{capabilities} of $\mathcal{Z}$ is specified as follows. 
\begin{description}
    \item[1] $\mathcal{Z}$ is able to choose inputs of the \textit{challenge protocols} and observes its outputs. (To specify, it can choose the inputs of the parties and observes the outputs obtained by the parties)
    \item[2] $\mathcal{Z}$ is able to interact with the attacker (which will be either the adversary $\mathcal{A}$ or the simulator $\mathcal{S}$)
\end{description}
The first capability models the behavior of other activity in the network that interacts with the \textit{challenge protocol} (for example, the \textit{challenge protocol} may be used as a subroutine or of another protocol).\par
The second capability models the the capability of the attacker to coordinate attacks based on information from other network activity.\par
A caveat is that \textit{the subroutine invoked by the challenge protocol is not allowed to interact with $\mathcal{Z}$}. We will discuss it later in Section~\ref{sec:GUC}. \par

Having the discussion above, we now provide a definition of security under basic UC framework. \par
\begin{definition}
    A protocol $\pi$ is a \textit{UC secure realization of an ideal functionality} if it \textit{UC emulates} the ideal functionality, in the sense that executing the protocol is indistinguishable for an external environment from an interaction with a trusted agent running the ideal functionality.
\end{definition}

In order to modular the protocol design, the concept if \textit{hybrid model} is introduced in basic UC framework.
\begin{definition}[Hybrid model]
    A protocol $\pi$ is said to be realized in the $\mathcal{G}$-hybrid model if $\pi$ invokes the ideal functionality $\mathcal{G}$ as a subroutine (it can also invoke $\mathcal{G}$ multiple times). We call $\mathcal{G}$ as \textit{subroutine ideal functionality of the protocol}.
\end{definition}

It also remains to consider security definition under hybrid model. We use $\mathcal{G}$-hybrid protocol to denote a protocol invoking ideal functionality $\mathcal{G}$ as subroutine.
\begin{definition}
    If a protocol $\pi$ is a \textit{UC secure realization of an ideal functionality}, and it is a $\mathcal{G}$-hybrid protocol, then we say that $\pi$ is a \textit{UC secure realization of the ideal functionality in the $\mathcal{G}$-hybrid model}.
\end{definition}

\subsubsection{Generalized UC framwork}\label{sec:GUC}
As suggested in previous section, the definition of UC security does not model the circumstance that a subroutine invoked by the \textit{challenge protocol} is also invoked by other protocol in the network. Namely, a protocol (which runs such a subroutine) proven to be UC secure might not 
actually secure in reality. Thus \cite{canetti2007universally} induces an enhanced definition of UC security, which takes the above issue into account.\par
To elaborate more on the difference, basic UC framework only models those "self-contained" protocols. This kind of protocol is defined as follows.
\begin{definition}[Subroutine respecting protocol]
    A protocol is said to be \textit{subroutine respecting} if it does not make use of \textit{subroutine ideal functionalities of other protocol sessions}.
\end{definition}

\begin{definition}[Shared ideal functionality]
    \textit{Shared ideal functionality} is a \textit{subroutine ideal functionality of the protocol $\pi$} that can be accessed by other protocol sessions. We denote \textit{shared ideal functionality} as $\overline{\mathcal{G}}$.
 \end{definition}

\begin{definition}[$\overline{\mathcal{G}}$-subroutine respecting protocol]
    A protocol $\pi$ is a \textit{$\overline{\mathcal{G}}$-subroutine respecting protocol} if $\pi$ only shares information via a single \textit{shared ideal functionality} $\overline{\mathcal{G}}$. 
\end{definition}

The security definition is similar to the definition of UC security. The main differences lies in follows:
\begin{description}
    \item[1] the use of unconstrained environment $\mathcal{Z}$
    \item[2] the ability of \textit{challenge protocols} $\pi$ and $\phi$ to invoke \textit{shared ideal functionality}
\end{description}
Notably, $\mathcal{Z}$ may essentially access shared functionalities by invoking other protocols which communicates with the shared functionalities. 


\begin{definition}
    A protocol $\pi$ is a \textit{GUC secure realization of an ideal functionality} if it \textit{GUC emulates} the ideal functionality, in the sense that executing the protocol is indistinguishable for an external environment from an interaction with a trusted agent running the ideal functionality.
\end{definition}

\begin{definition}
    If a protocol $\pi$ is a \textit{GUC secure realization of an ideal functionality}, and it is a $\mathcal{G}$-hybrid protocol, then we say that $\pi$ is a \textit{GUC secure realization of the ideal functionality in the $\mathcal{G}$-hybrid model}.
\end{definition}

\subsubsection{Details of real world/ideal world comparison}

\iffalse
\begin{definition}[Environment]
The \textit{environment} is essentially a distinguisher who intends to distinguish whether he is interacting with real-world protocol or ideal-world functionality. The environment interacts with the protocol as follows\footnote{For simplicity, we abuse the notation and call the simulator in ideal world as adversary.}:\par
\begin{description}
    \item[1] Before the execution starts, the environment hands arbitrary inputs chosen by him to the parties and the adversary.
    \item[2] During protocol execution, the environment and the adversary
are allowed to interact at any point throughout the course of protocol execution (in particular, they can exchange information).
    \item[3]  Once the execution terminates, the environment collects the outputs from the parties and the adversary. 
    \item[4] Finally the environment outputs a single bit which represents whether he thinks he has interacted with the protocol $\Pi$, or the ideal functionality.
\end{description}
\end{definition}
\fi

In ideal world, there is an ideal functionality $\mathcal{F}$ and dummy parties. Upon receiving an inputs from $\mathcal{Z}$, a dummy party forwards the input to $\mathcal{F}$; upon receiving an output from $\mathcal{F}$, a dummy party forwards this value to $\mathcal{Z}$. Simulator can communicate directly with $\mathcal{F}$, and sends messages to environment $\mathcal{Z}$.\par
In real world, we only cover semi-honest adversary here. All the parties execute the protocol $\Pi$. The environment $\mathcal{Z}$ writes inputs to all the parties and reads the subrountine outputs of parties. During the whole execution, $\mathcal{Z}$ and $\mathcal{A}$ can interact. $\mathcal{A}$ may read the outputs of all parties. Note that parties may have subroutines to which $\mathcal{Z}$ has no direct access.\par


\iffalse
Security of protocols is defined by way of comparing the real-world protocol execution to an ideal process for carrying out the prescribed tasks. Namely, we compare a concrete real-world protocol to an ideal protocol that make use of \textit{ideal functionality} who acts as a trusted center that captures all the desired tasks we want to achieve. 
For example, the definition of semantic security for encryption compares what can be learned by an adversary who receives a real ciphertext to what can be learned by an adversary who receives nothing. The definition of security states that an encryption scheme is secure if they can both learn approximately the same amount of information.\par

\begin{definition}[Ideal process]
All parties hands in their inputs to a trusted agent who internally computes the outputs, and hand each party its prescribed output.
\end{definition}

\begin{definition}[Ideal functionality]
The trusted agent in ideal process is modeled as ideal functionality who is repeatedly receiving inputs from the parties and provides them with appropriate outputs, while maintaining local state in between.
\end{definition}



\textit{Simulation} is how we prove security under the above cryptographic notion. To specify, if for every adversary in real-world execution, there exists s simulator in ideal world, that a environment $\mathcal{Z}$ cannot distinguish between these two world, then the real-world protocol is secure. A simulator essentially simulates the behavior of real-world adversary, trying to generate messages during the execution, and make the ideal-world execution almost the same with real-world execution from the perspective of environment $\mathcal{Z}$.

\begin{definition}
A real-world protocol $\Pi$ is said to securely realize ideal functionality $\mathcal{F}$
if for any real-world adversary $\mathcal{A}$ (who interacts with $\mathcal{Z}$) and real players executing $\Pi$, there exists an ideal-world simulator $\mathcal{S}$ (who interacts with $\mathcal{Z}$ and $\mathcal{F}$) and the dummy parties communicating with $\mathcal{F}$, such that no probabilistic polynomial time environment $\mathcal{Z}$ can tell whether it is interacting with 
$\mathcal{A}$ or with $\mathcal{S}$, except with negligible probability.
\end{definition}
\fi


\section{Formal security proof: Sktech}
\begin{assumption}\label{assume: asm}
    The encryption scheme is IND-CPA secure symmetric encryption, the commitment scheme is substituted by hash function modeled as random oracle (as suggested in \cite{dziembowski2018fairswap}), all the parties are polynomial time bounded. Messages sent between buyer and receiver is through a secure point-to-point channel. There is no external parties who interacts with sellers during MPC phase.
\end{assumption}

\begin{theorem}
    Under Assumption~\ref{assume: asm}, Smart MPC-PP protocol is a \textit{GUC secure realization of an ideal functionality $\mathcal{F}$} in the $(\mathcal{J} , \mathcal{H}, \mathcal{M})$-hybrid model except with negligible probability, where $\mathcal{F}, \mathcal{J}, \mathcal{H}, \mathcal{M}$ are defined as follows.
\end{theorem}
We defer the full proof in Section~\ref{sec:full}.

\begin{theorem}
    Under Assumption~\ref{assume: asm}, Smart MPC-PP protocol is a \textit{GUC secure realization of an ideal functionality $\mathcal{F}$} in the $(\mathcal{J} , \mathcal{H})$-hybrid model except with negligible probability.
\end{theorem}

\begin{proof}
    There exists two-party protocols and multi-party protocols which are universally composable \cite{canetti2002universally}, and according to assumption~\ref{assume: asm}, it \textit{GUC secure realize $\mathcal{F}$} in the $(\mathcal{J}, \mathcal{H})$-hybrid model.
\end{proof}


\section{Formal security proof: full version}\label{sec:full}
\subsection{Definition of ideal functionalities in our scenario}

%real world/ideal world

%UC...environment


%define ideal world/real world


Define the functionality of $\mathcal{J}$:
\begin{description}
    \item Upon receiving $\texttt{Com}(\pi_1(Q)) , \texttt{Com}(\pi_2(Q))$ from buyer, store, and sends them to sellers
    \item Upon receiving $\texttt{Com}(\enc_{\text{info-key}_1}(\text{info}_1)), \texttt{Com}(\enc_{\text{info-key}_2}(\text{info}_2))$, store, sends them to buyer
    \item Upon receiving $\texttt{Com}(\text{info-key}_1)， \texttt{Com}(\text{info-key}_2)$, store
    \item Upon receiving $\text{info-key}_1, r_5;\text{info-key}_2, r_6 $, checks, if verification fails, terminate.
    \item Upon receiving $o_1, o_2$, allocates money.
\end{description}

Define the functionality of $\mathcal{M}$:
\begin{description}
    \item Upon receiving $\text{info}_1, \text{info}_2$, outputs $o_1, o_2$ where $o_1 = o_2 = \textsc{PayFunc}(\text{info}_1, \text{info}_2)$.
\end{description}








According to the definition of ITP in Definition ~\ref{def:itp},
$\mathcal{F}$ is an ideal functionality of ITP; Smart MPC-PP protocol is a real-world protocol for ITP. We will prove in the following that Smart MPC-PP securely realizes the ideal functionality $\mathcal{F}$.\par

In order to provide readers with a more clear view, we first informally describes the ideal functionality $\mathcal{F}$, and then give the formal definition.\par

\begin{description}
    \item[1] Buyer and seller agree upon coefficients and MI function, send them to $\mathcal{F}$. $\mathcal{F}$ checks whether these things are consistent, if not, terminates.
    \item[2] Buyer submit question set to $\mathcal{F}$, $\mathcal{F}$ generate two random orders, sends questions (arranged by random orders) to sellers respectively.
    \item[3] After sellers finish questions, they send their info (question set and corresponding answers) to $\mathcal{F}$, then $\mathcal{F}$ checks the whether the question sets submitted by sellers are indeed the questions that buyer previously provided. If not, terminates (and allocate fine)
    \item[4] $\mathcal{F}$ computes \textsc{PayFunc}. 
    \item[5] $\mathcal{F}$ allocates money according to the payment function.
\end{description}

\subsection{Simulation}
\begin{proof}

We denote the simulator as Sim.\par

    Sim learns question set from $\mathcal{F}$.\par
    
    Sim selects two random permutations $\pi_1', \pi_2'$ and permutes $Q$ to obtain $\pi_1'(Q), \pi_2'(Q)$\par
    
    Sim committed to these two permuted question sets, and gets $\texttt{Com}(\pi_1'(Q)), \texttt{Com}(\pi_2'(Q))$
    and opening information $r_1', r_2'.$\par
    
    Sim simulates the real-world protocol $\Pi$ by running $\mathcal{J}(\texttt{Com}(\pi_1'(Q)), \texttt{Com}(\pi_2'(Q)))$.\par
    
    Sim sends [$r_i', \pi_i'(Q)$] to sellers and let sellers check whether the permuted question set is buyer previously committed to. If not, Sim terminates the simulation.\par
    
    % Above simulation is perfect.
    
    Sim packages info of sellers as $ \pi_i'(Q)\| 0^n$, 
    generates $\text{info-key}_i$ and 
    encrypts it and gets $\enc_{\text{info}_i}(\text{info}_i)$.\par
    
    Sim commits to the $\enc_{\text{info}_i}(\text{info}_i)$ to get $\texttt{Com}(\enc_{\text{info}_i}(\text{info}_i))$ and $r_3', r_4'$, \\
    then run $\mathcal{J}(\texttt{Com}(\enc_{\text{info}_1}(\text{info}_1)), \texttt{Com}(\enc_{\text{info}_2}(\text{info}_2)))$ to simulate $\Pi$.\par
    
    Sim sends $\enc_{\text{info}_1}(\text{info}_1), r_3' ; \enc_{\text{info}_i}(\text{info}_i), r_4'$ to buyer, and buyer checks whether the $\enc_{\text{info}_i}(\text{info}_i)$ is what sellers previously committed to. If not Sim terminates the simulation.\par
    
    Sim commits to $\text{info-key}_i$ and gets $\texttt{Com}(\text{info-key}_1), r_5'; \texttt{Com}(\text{info-key}_2), r_6'$.\\
    Run $\mathcal{J}(\texttt{Com}(\text{info-key}_1), \texttt{Com}(\text{info-key}_2))$ to simulate the key committing phase.\par
    
    Sim calls $\mathcal{M}(\text{info}_1, \text{info}_2)$ to simulate MPC phase in real world, and gets outputs $o_1, o_2$.\par
    
    Upon receiving $\text{info-key}_i$ from $\mathcal{F}$, Sim calls $\mathcal{J}(\text{info-key}_1, r_5'; \text{info-key}_2, r_6')$ to simulate the behavior of $\mathcal{J}$ (in this phase $\mathcal{J}$ checks info-key, sends info-key to buyer). If $\mathcal{J}$ terminates, then Sim terminates the simulation.\par
    
    Sim calls $\mathcal{J}(o_1,o_2)$ to simulate the transaction phase. (During which $\mathcal{J}$ allocates the money)\par
    
    Sim terminates.\par


The simulation will only fail if $\mathcal{Z}$ learns $\enc_{\text{info-key}_i} (\pi_i'(Q) \| 0^n)$
and decrypts them to $\pi_i'(Q)\|0^n$, and in this case $\mathcal{Z}$ will distinguish between these two execution. This will only happen with negligible probability when the hinding property of commitment scheme (constructed by hash) is broken.\par

\end{proof}


\iffalse
\begin{lemma} (Sequential Composition)
Let $g_i$ denote ideal functionality, and let $\Pi^{\rho_1,...}$ denote the real world protocol such that 1) sub-protocol $\rho_1,...$ are called sequentially, 2) no $\Pi$-messages sent while $\rho_1, ... $ are executed. If $\Pi^{g_1,...}$ is a secure hybrid world protocol computing $f$ and each $\rho_i$ securely computes $g_i$, then $\Pi^{\rho_1,...} $ is a secure real-world protocol computing $f$.  
\end{lemma}

We have proved that our Smart-MPC-PP protocol is a secure hybrid world protocol 
that realizes the ideal functionality $\mathcal{F}$ under the above assumption, then using the sequential composition theorem (where $\rho_i$ is real-world MPC protocol
and $g_i$ is ideal functionality in MPC, and MPC is universally composable \cite{canetti2002universally}) to show that our Smart-MPC-PP protocol
is a secure real-world protocol.\par
\fi

\iffalse
\subsubsection{Basic definitions}
In this section, we provide formal definitions related to cryptographic primitives used in our protocol.

\begin{definition}(negligible function)\par
A function $\mu: \mathbbm{N} \rightarrow \mathbbm{R}$ is \textit{negligible} iff $ \forall c\in \mathbbm{N}, \exists n_0 \in \mathbbm{N} $ such that $\forall n\ge n_0, \mu(n)\le n^{-c}$.
\end{definition}
Intuitively speaking, a negligible function approaches zero
asymptotically faster than any inverse polynomial.\par

\begin{definition}(computational indistinguishablilty)\par
For two sequences of distributions $\{A_n\}, \{B_n\}$ where $A_n, B_n$ ranging over $\{0,1\}^{l(n)}$ for some $l(n) = n^{O(1)}$. Then $\{A_n\} , \{B_n\}$ are \textit{computationally indistinguishable} if for every polynomial time distinguisher $D$, 
$$ |\Pr_{x\leftarrow A_n}[D(x)=1] - \Pr_{x\leftarrow B_n}[D(x)=1]|\le \mu(n)$$
We denote it as $\{A_n\}\approx_c \{B_n\}.$
\end{definition}


\subsubsection{Basic primitives}
In this section we provide the main cryptographic primitives used in our protocol and briefly discuss their properties, and omit the details.\footnote{For succinctness, the description in this section may not be fully rigorous in standard cryptographic prospective, but is sufficient in our scenario.}\par
\begin{definition}hash function\par
A hash function $\hash : \{0,1\}^* \leftarrow \{0,1\}^{\mu}$ maps an arbitrary length binary strings to a string of a fixed length $\mu$. 
\end{definition}

\begin{definition}(collision resistance)\par
A set of functions $H = \{h_i : D_i \rightarrow R_i\}_{i\in I}$ is a family of \textit{collision resistant hash functions} if\par
\begin{itemize}
    \item (easy to sample) there exists a PPT algorithm Gen s.t. $\text{Gen}(1^n) \in I$
    \item (compress) $|R_i| < |D_i|$
    \item (easy to evaluate) there is a PPT algorithm Eval s.t. $\forall x\in D_i$ and $\forall i\in I$, $\text{Eval}(x,i)= h_i(x)$
    \item (collision resistant) $\forall $ non-polynomial adversary $\mathcal{A}$, there is a negligible function $\mu$ s.t. for $n\in \mathbbm{N}$
    $$ \Pr[x_1\ne x_2 \wedge h_i(x_1)=h_i(x_2)\ |\ i\leftarrow \text{Gen}(1^n), (x_1,x_2)\leftarrow \mathcal{A}(1^n,i)] \le \mu(n)$$
    
\end{itemize}
\end{definition}

Loosely speaking, for collision resistant hash functions, it should be difficult to find two messages $m_1,m_2$ such that $\hash(m_1) = \hash(m_2)$.
 For provable security reason, in this work we model it as random oracle\footnote{Here is the explanation of random oracle model}.\par

\ym{need to define encryption scheme?}

\begin{definition}indistinguishability under chosen ciphertext attack (IND-CPA)\par
Let $\mathcal{E} = (\text{Gen}, \enc, \dec)$ be a symmetric encryption scheme, and let $\mathcal{A}$ be an polynomial adversary who has access to an oracle. We consider the following two experiments:\par
$\textbf{Expt}_{\mathcal{A}}^0 : k\leftarrow \text{Gen}(1^n), b\leftarrow \mathcal{A}^{LR(\cdot, \cdot, 0)}, \text{return } b$\par

$\textbf{Expt}_{\mathcal{A}}^1 : k\leftarrow \text{Gen}(1^n), b\leftarrow \mathcal{A}^{LR(\cdot, \cdot, 1)}, \text{return } b $\par
Then $\mathcal{E}$ is IND-CPA secure encryption scheme if 
$$ |Pr[\textbf{Expt}_{\mathcal{A}}^0 =1] - \Pr[\textbf{Expt}_{\mathcal{A}}^1 =1 ] |\le \mu(n)$$
\end{definition}
Intuitively speaking, IND-CPA secure symmetric encryption guarantees that the encryption of two strings is indistinguishable, and further, an adversary (e.g. an eavesdropper in the communication channel between buyer and sellers) cannot distinguish the ciphertext of $m_0, m_1$ chosen by her in any case.
\par
\fi



\iffalse
\begin{definition}[indistinguishability under chosen ciphertext attack (IND-CPA)]\par

Let $\mathcal{E} = (\text{Gen}, \enc, \dec)$ be a symmetric encryption scheme, and let $\mathcal{A}$ be an polynomial adversary who has access to an $\mathcal{E}_k(LR(\cdot,\cdot, b))$ oracle.
The oracle $\mathcal{E}_k(LR(\cdot,\cdot, b))$ on receiving an input $(m_0,m_1)$, computes $c\leftarrow \enc_{k}(m_b)$, and outputs $c$. We consider the following two experiments:\par
$\textbf{Expt}_{\mathcal{A}}^0 : k\leftarrow \text{Gen}(1^n), b\leftarrow \mathcal{A}^{\mathcal{E}_k(LR(\cdot, \cdot, 0))}, \text{return } b$\par

$\textbf{Expt}_{\mathcal{A}}^1 : k\leftarrow \text{Gen}(1^n), b\leftarrow \mathcal{A}^{\mathcal{E}_k(LR(\cdot, \cdot, 1))}, \text{return } b $\par
Then $\mathcal{E}$ is IND-CPA secure encryption scheme if 
$$ |Pr[\textbf{Expt}_{\mathcal{A}}^0 =1] - \Pr[\textbf{Expt}_{\mathcal{A}}^1 =1 ] |\le \mu(n)$$
\end{definition}
\fi


==> other.tex <==

\begin{description}
\item[Step 1: Sign contract] The buyer and two sellers agree on two coefficients $\alpha,\beta\geq 0$ and sign a contract: if the output of protocol MPC-PP is $(\text{success},v)$, the buyer transfers $\frac{\alpha v+\beta}{2}$ to both the two sellers; otherwise the contract ends.

\item[Step 2: Questions assignment] The buyer prepares a private random order $\mathbf{o}$ of the $n$ events (e.g. $n=3$, possible $\mathbf{o}=\{1,3,2\}$) and assigns the events to the first seller according to the original order and the events to the second seller according to the random order $\mathbf{o}$, with an opinion format. 

\item[Step 3: Protocol MPC-PP$\left(F(\mathbf{u}_A,\mathbf{u}_B,\mathbf{o})\right)$] The buyer and two sellers run MPC-PP to compute function $F(\mathbf{u}_A,\mathbf{u}_B,\mathbf{o})$ where $\mathbf{u}_A,\mathbf{u}_B$ are two sellers' reports respectively and $\mathbf{o}$ is the buyer's random order, where 
$$ F(\mathbf{u}_A,\mathbf{u}_B,\mathbf{o}) := \begin{cases}
MIG^{tvd}(\pi_{\mathbf{o}} \mathbf{u}_A,\mathbf{u}_B)& \mathbf{u}_A,\mathbf{u}_B\in \Sigma^n\\
MIG^{Pearson}(\pi_{\mathbf{o}} \mathbf{u}_A,\mathbf{u}_B; \mathbf{p})& \mathbf{u}_A,\mathbf{u}_B\in {\Delta_{\Sigma}}^n \end{cases} $$
\end{description}


\begin{align} \label{eq:mig}
    MIG^{tvd}(\mathbf{u}_A,\mathbf{u}_B)=&\frac{1}{n}\sum_{i} \mathbbm{1}(\mathbf{u}_A(i)==\mathbf{u}_B(i)) \\ \nonumber
    &-\frac{1}{n(n-1)}\sum_{i\neq j}\mathbbm{1}(\mathbf{u}_A(i)==\mathbf{u}_B(j))
\end{align}

\begin{align} \label{eq:mig}
    MIG^{Pearson}(\mathbf{u}_A,\mathbf{u}_B;\mathbf{p})=&\frac{1}{n}\sum_{i} 2\bigg(\sum_{\sigma \in\Sigma }\frac{ \mathbf{u}_A(i)_{\sigma} \cdot \mathbf{u}_B(i)_{\sigma} }{\mathbf{p}_{\sigma}}-1\bigg)\\ \nonumber
    &-\frac{1}{n(n-1)}\sum_{i\neq j}\Bigg(\bigg(\sum_{\sigma\in\Sigma} \frac{\mathbf{u}_A(i)_{\sigma} \cdot \mathbf{u}_B(j)_{\sigma}}{\mathbf{p}_{\sigma}}\bigg)^2-1\Bigg) 
\end{align}

==> otherpp.tex <==
\subsubsection{Correlation-PP: unverifiable signals elicitation}\label{sec:corrpp}
Alice and Bob are assigned $n$ a priori similar questions (e.g. medical image labeling questions). For each question $i$, Alice and Bob receive private signals $\sigma_A^i\in\Sigma$ and $\sigma_B^i$ respectively (e.g. good/bad). We say Alice and Bob report honestly if they reports their private signals. 

\begin{assumption}[A priori similar and random order]
    All questions have the same prior. All questions appear in a random order, independently drawn for both Alice and Bob.
\end{assumption}

Correlation-PP also requires an additional \emph{positively correlated} assumption that assumes that Alice and Bob's private signals are positively correlated. Correlation-PP also requires several mild conditions on the prior, i.e., the joint distribution over Alice and Bob's private signals. We omit the formal definitions here as it's not the focus of this paper. Interested readers are referred to \citet{2016arXiv160303151S,2016arXiv160501021K} 

\paragraph{Correlation-PP}\cite{2016arXiv160303151S,2016arXiv160501021K}
\begin{description} 
\item[Report] for each question $i$, Alice is asked to report $\sigma_A^{i}$ and Bob is asked to report $\sigma_B^{i}$. We denote Alice and Bob's honest report for all questions by $\mathbf{\sigma}_A$ and $\mathbf{\sigma}_B$ respectively and denote their actual reports by $\hat{\mathbf{\sigma}}_A$ and $\hat{\mathbf{\sigma}}_B$. 

\item[Payment] Alice and Bob are rewarded by the average ``the amount of agreement'' between their forecasts in \emph{same} task, and punished the average ``the amount of agreement'' between their forecast in \emph{distinct} tasks, i.e., 
\begin{align} \label{eq:mig}
    MIG^{Corr}(\mathbf{\sigma}_A,\mathbf{\sigma}_B)=&\frac{1}{n}\sum_{i} \bigg(\mathbbm{1}(\sigma_A^i==\sigma_B^i)\bigg)\\ \nonumber
    &-\frac{1}{n(n-1)}\sum_{i\neq j}\bigg(\mathbbm{1}(\sigma_A^i==\sigma_B^i)\bigg)
\end{align}
\end{description}

Alice and Bob play a \emph{permutation strategy profile} if they both report the same permutation of their honest signals. (e.g. they say good when it's bad and say bad when it's good).

\begin{lemma}[Correlation-PP is truthful]\cite{2016arXiv160303151S,2016arXiv160501021K}\label{lem:corr}
With positively correlated assumption, and a priori similar and random order assumption, and mild conditions on the prior, Correlation-PP has truth-telling is a strict equilibrium and also the best equilibrium in the sense that each agent's expected payment is strictly maximized if agents tell the truth or play a permutation strategy profile.
\end{lemma}


\subsubsection{Pearson-PP: unverifiable forecasts elicitation}\label{sec:pearsonpp}

Alice and Bob are assigned $n$ a priori similar forecasting tasks. For each forecasting task $i$, Alice's private information is $x_A^{i}$ and Bob's private information is $x_B^{i}$, both of them are asked to forecast the outcome $y^{i}\in\Sigma$ of the event $Y$ in task $i$ (e.g. the pathological truth of the medical image).

\begin{assumption}[A priori similar and random order]
    For each task $\ell$, fresh i.i.d. realizations of $(X_A,X_B,Y)=(x_A^{\ell},x_B^{\ell},y^{\ell})$ are generated. All tasks appear in a random order, independently drawn for both Alice and Bob.
\end{assumption}

Pearson-PP also requires an additional \emph{conditional independent} assumption that assumes that Alice and Bob's private information are independent conditioning on the realization of the event $Y$. 

\begin{definition}[truthful strategy in forecasting tasks]
Alice reports honestly iff for every task $i$, she reports her Bayesian posterior $\mathbf{p}_A^{i}\in\Delta_{\Sigma}$ where $\mathbf{p}_A^{i}(y):=\Pr[Y=y|X_A=x_A^{i}],\forall y\in\Sigma$. We have similar definition for Bob.  
\end{definition}

Informally, Alice and Bob play a \emph{permutation strategy profile} if they both permute the outcomes and report the permuted version (e.g. their honest forecasts are 70\% benign, 30 \% malignant and 65\% benign, 35\% malignant but they instead report  30\% benign, 70 \% malignant and 35\% benign, 65\% malignant). Moreover, like Correlation-PP, Pearson-PP also requires several mild conditions on the prior, i.e., the joint distribution over Alice and Bob's private information and the event $Y$. We omit the formal definitions here and interested readers are referred to \citet{kong2018water}.


\paragraph{Pearson PP}\cite{kong2018water} Given the prior distribution over $Y$ $\Pr(Y=y),\forall y$, 
\begin{description} 
\item[Report] for each task $i$, Alice is asked to report $\mathbf{p}_A^{i}$ and Bob is asked to report $\mathbf{p}_B^{i}$. We denote Alice and Bob's honest report for all tasks by $\mathbf{p}_A$ and $\mathbf{p}_B$ respectively and denote their actual reports by $\hat{\mathbf{p}}_A$ and $\hat{\mathbf{p}}_B$. 

\item[Payment] The payment has the same spirit with Correlation PP's payment, with more delicate ``amount of agreement'':
\begin{align} \label{eq:mig}
    MIG^{Pearson}(\mathbf{p}_A,\mathbf{p}_B)=&\frac{1}{n}\sum_{i} 2\bigg(\sum_{y\in\Sigma}\frac{\mathbf{p}_A^i(y) \mathbf{p}_B^i(y)}{\Pr[Y=y]}-1\bigg)\\ \nonumber
    &-\frac{1}{n(n-1)}\sum_{i\neq j}\Bigg(\bigg(\sum_{y\in\Sigma}\frac{\mathbf{p}_A^i(y) \mathbf{p}_B^i(y)}{\Pr[Y=y]}\bigg)^2-1\Bigg) 
\end{align}
\end{description}

\begin{lemma}[Pearson-PP is truthful]\cite{kong2018water}\label{lem:pearson}
With the conditional independence assumption, and a priori similar and random order assumption, and mild conditions on the prior, given the prior distribution over the $Y$, Pearson-PP has truth-telling is a strict equilibrium and also the best equilibrium in the sense that each agent's expected payment is strictly maximized if agents tell the truth or play a permutation strategy profile.
\end{lemma}



==> smart_formal.tex <==

\begin{table}[htb]%\resizebox{1.4\textwidth}
	\caption{Protocol: buyer and sellers}
	\label{protocol:TCbuyerseller}
	\begin{minipage}{\columnwidth}
		\begin{center}
%			\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}}
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}}
				\toprule
				\textbf{Sign smart contract}\\
	            Buyer and two sellers:\\
	            \qquad select the coefficients of the payment function\\ 
	            \qquad commit the coefficients to the public\\
	            \qquad commit the MI function to the public\\
				\hline
				\textbf{Assign questions}\\
				$\mathcal{B}$:\\
				\qquad $o_{\mathcal{S}_1}, o_{\mathcal{S}_2} \leftarrow \text{Gen}(1^{\kappa})$\\
				\qquad $ id_{\mathcal{S}_1}, id_{\mathcal{S}_2} \leftarrow \text{Gen}(1^{\rho})$\\
				
				\qquad{sends $(id_{\mathcal{S}_i},\ o_{\mathcal{S}_i} \circ Q_\mathcal{B})$ to $\mathcal{S}_i$}\\
				
				\qquad Upon receiving $c_{\mathcal{S}_0}^{info}, c_{\mathcal{S}_1}^{info}$\\
				\qquad store them locally\\
				
				
				$\mathcal{S}_i:$\\
				\qquad Upon receiving $(id_{\mathcal{S}_i},\ Q_{\mathcal{S}_i})$\\
				\qquad $com_{\mathcal{S}_i}^{iq} \leftarrow \hash(id_{\mathcal{S}_i},\ Q_{\mathcal{S}_i}) $\\
				\qquad sends $com_{\mathcal{S}_i}^{iq}$ to $\mathcal{J}$\\
				
				\qquad $ans_{\mathcal{S}_i} \leftarrow  \text{Ans}_{\mathcal{S}_i} (Q_{\mathcal{S}_i})$\\
				
				\hline
				\textbf{Finish Questions}\\
				$\mathcal{S}_i:$\\
				\qquad $info_{\mathcal{S}_i} := (id_{\mathcal{S}_i}, Q_{\mathcal{S}_i}, ans_i)$\\
				\qquad $\textsc{Kinfo}_{\mathcal{S}_i} \leftarrow \text{Gen}(1^l), \ \textsc{Kcon}_{\mathcal{S}_i}\leftarrow \text{Gen}(1^m)$\\
				\qquad $c_{\mathcal{S}_i}^{info} \leftarrow \enc_{\textsc{Kinfo}_{\mathcal{S}_i}}(info_{\mathcal{S}_i})$\\
			
				
				\qquad $com_{\mathcal{S}_i}^{ei} \leftarrow \hash (c_{\mathcal{S}_i}^{info})$\\
				
				\qquad $c_{\mathcal{S}_i}^k \leftarrow
				\enc_{\textsc{Kcon}_{\mathcal{S}_i}}(\textsc{Kinfo}_{\mathcal{S}_i})$\\
				\qquad sends $c_{\mathcal{S}_i}^{info}$ to $\mathcal{B}$\\
				\qquad sends $com_{\mathcal{S}_i}^{ei} $ to $\mathcal{J}$\\
				\qquad sends $c_{\mathcal{S}_i}^k$ to $\mathcal{J}$\\
				
				%\hfill {$\blacktriangleright$ \emph{avoid the trusted center to get the information outside of rebuttal}}\\
				
				
				\hline
				\textbf{MPC}\\
			
				$\mathcal{S}_0, \mathcal{S}_1$ run 2PC protocol $\mathcal{P}(function((com_{\mathcal{S}_1}^{ei},info_{\mathcal{S}_0}, \textsc{Kinfo}_{\mathcal{S}_0}), (com_{\mathcal{S}_0}^{ei}, info_{\mathcal{S}_1}, \textsc{Kinfo}_{\mathcal{S}_1})))$ \\
				to get $out_i$ for $\mathcal{S}_i$, 
				where $out_i=val $ or \texttt{abort}\\
				
				
				$\mathcal{S}_i:$ 
				 sends $out_i$ to $\mathcal{J}$\\
				\bottomrule
			\end{tabular*}
		\end{center}
		\bigskip\centering
%		\footnotesize\emph{Source:} This is a table
%		\emph{Note:} This is a table footnote.
	\end{minipage}

\end{table}

\begin{table}[htb]%\resizebox{1.4\textwidth}
	\caption{Protocol: buyer and sellers, continued}
	\label{protocol:TCbuyerseller}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}}
				\toprule
				\textbf{Check}\\
				$\mathcal{S}_i:$ \\
				\qquad sends $\textsc{Kcon}_{\mathcal{S}_i}$ to $\mathcal{J}$\\
				
				$\mathcal{B}:$\\
				\qquad $k_{\mathcal{B}}\leftarrow \dec_{\textsc{Kcon}_{\mathcal{S}_i}}(\textsc{Kinfo}_{\mathcal{S}_i})$, where $k_{\mathcal{B}}$ is $\perp $ or valid\\
				\qquad $m_{\mathcal{B}} \ \leftarrow \dec_{\textsc{Kinfo}_{\mathcal{S}_i}}(c_{\mathcal{S}_i}^{info})$, where $m_{\mathcal{B}} $ is $\perp$ or $(id_{\mathcal{S}_i}, Q_{\mathcal{S}_i}, ans_{\mathcal{S}_i})$\\
				\qquad \texttt{if} $k_{\mathcal{B}}$ is $\perp$ or $m_{\mathcal{B}}$ is $\perp$ or any of $(id_{\mathcal{S}_i}, Q_{\mathcal{S}_i}, ans_{\mathcal{S}_i}) $ is incorrect or not consistent with MI\\
				\qquad \qquad goto \textbf{Rebuttal}\\
				
				\hline
				\textbf{Rebuttal}\\
				$\mathcal{B}$:\\
				\qquad sends $c_{\mathcal{S}_0}^{info}, c_{\mathcal{S}_1}^{info}$ to $\mathcal{J}$\\
				\bottomrule
			\end{tabular*}
		\end{center}
		\bigskip\centering
%		\footnotesize\emph{Source:} This is a table
%		\emph{Note:} This is a table footnote.
	\end{minipage}

\end{table}


\begin{table}[htb]%\resizebox{1.4\textwidth}
	\caption{Protocol: smart contract $\mathcal{J}$}
	\label{protocol:TCbuyerseller}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}}}
				\toprule
				\textbf{Check}\\
				Upon receiving $  out_i$ for $i=1,2$, \\
				\texttt{if} exists $i $ s.t. $out_i$ is \texttt{abort}\\
				\qquad takes all sellers deposits, return buyer's deposits and terminates\\
				\texttt{else if} $out_0$ equals to $out_1$\\
				\qquad waits for \textbf{Rebuttal} (if no such message received, make transactions, terminates)\\
				\texttt{else} takes all sellers' deposits, return buyer's deposits and terminate\\
				
				\hline
				\textbf{Rebuttal}\\
				Upon receiving $( c_{\mathcal{S}_0}^{info},c_{\mathcal{S}_1}^{info} )$ from $\mathcal{B}$\\
			    computes $(chk_0, chk_1) \leftarrow (\hash(c_{\mathcal{S}_0}^{info}),\hash(c_{\mathcal{S}_1}^{info}))$ \\
				\texttt{if} $(chk_0, chk_1)$ is inconsistent with $(com_{\mathcal{S}_0}^{ei}, com_{\mathcal{S}_1}^{ei})$, $\mathcal{J}$ takes all the money\\
				
				$k_\mathcal{J} \leftarrow \dec_{\textsc{Kcon}_{\mathcal{S}_i}}(\textsc{Kinfo}_{\mathcal{S}_i})$\\
				$m_{\mathcal{J}}\leftarrow \dec_{\textsc{Kinfo}_{\mathcal{S}_i}}(c_{\mathcal{S}_i}^{info})$ \\
				parse $m_\mathcal{J} := (id_{\mathcal{S}_i}, Q_{\mathcal{S}_i}, ans_{\mathcal{S}_i})$\\
				
				\texttt{if} $k_{\mathcal{J}}$ or $m_{\mathcal{J}}$ is $\perp$\\
				\qquad rebuttal succeeds, give all the deposits to buyer\\
				
				
				\texttt{else}\\
				\qquad computes $ \hash(\enc_{\textsc{Kinfo}_{\mathcal{S}_i}} (id_{\mathcal{S}_i}, Q_{\mathcal{S}_i}))$ and $MI((Q_{\mathcal{S}_0}, ans_{\mathcal{S}_0}),(Q_{\mathcal{S}_1}, ans_{\mathcal{S}_1}))$ \\
				\qquad and check whether they are consistent with $com_{\mathcal{S}_i}^{iq}$ and $out_i$\\
			    \qquad \texttt{if} inconsistent \\
				\qquad \qquad rebuttal succeeds, give all deposits to $\mathcal{B}$\\
				\qquad \texttt{else} \\
				\qquad \qquad rebuttal fails, give all deposits to sellers (how sellers share the money???)\\
				
				
				\bottomrule
			\end{tabular*}
		\end{center}
		\bigskip\centering
%		\footnotesize\emph{Source:} This is a table
%		\emph{Note:} This is a table footnote.
	\end{minipage}

\end{table}



%\yk{where to define data/info?}
%\yk{what is $m$?}
%\yk{buyer also sends question set to tc} \yk{problem of hash: hash short information}


